A Systematic Analysis of Large Language Models as Soft Reasoners: The Case of Syllogistic Inferences

The reasoning abilities of Large Language Models (LLMs) are becoming a central focus of study in NLP. In this paper, we consider the case of syllogistic reasoning, an area of deductive reasoning studied extensively in logic and cognitive psychology. Previous research has shown that pre-trained LLMs exhibit reasoning biases, such as $\textit{content effects}$, avoid answering that $\textit{no conclusion follows}$, display human-like difficulties, and struggle with multi-step reasoning. We contribute to this research line by systematically investigating the effects of chain-of-thought reasoning, in-context learning (ICL), and supervised fine-tuning (SFT) on syllogistic reasoning, considering syllogisms with conclusions that support or violate world knowledge, as well as ones with multiple premises. Crucially, we go beyond the standard focus on accuracy, with an in-depth analysis of the conclusions generated by the models. Our results suggest that the behavior of pre-trained LLMs can be explained by heuristics studied in cognitive science and that both ICL and SFT improve model performance on valid inferences, although only the latter mitigates most reasoning biases without harming model consistency.

==> conclusion_notes.tex <==
\section{Conclusion and Future Research}

\tb{Example of we know humans weakness and aim to make models overcome such weakness so to help humans on their weak points}

\tb{cite ~\cite{ijcai2020p537} transformers are soft reasoner (Roberta trained on reasoning from facts and rules answer questions that needs the rules to be applied to the facts.)}

\rb{By minimizing errors in next-word prediction models learn a language. It's not known yet which is the right method to elicit or inject reasoning skills into LMs.  ICL has been claimed to elicit reasoning ability and avoid the risk to overfit proper of Fine-tuning. Our results show that indeed ICL are a powerful method to elicit reasoning yet dynamic it seems to be a promising method to  inject reasoning skills into LMs while avoiding the risk to overfit}

\tb{\cite{wu-etal-2023-hence} benchmark with other types of syllogisms, e.g. hypothetical, disjunction.. we could extend the work}

\tb{current attention is on bootstrapping methods to obtain data to train models, with logical reasoning this is not necessary: few clear rules. The challenge is to learn the abstract schema and apply them to all instances syntatically}

\paragraph{Future} In future works ...

\tb{future challenge: compose schemas, use schema within problems expressed with linguistically richer expressions, reduce a wordy problems to the schema}

\tb{connection with~\cite{yang:llm24} LLMs latently perform multi-hop reasoning. In our case, the latent chain is not of facts stored in the parameters rather in an intermediate conclusion inferred from a subset of premises.}

\tb{recursivity and compositionality}
We have tested the models on unseen content, and on unseen figure, but how useful it is to master syllogism?

\tb{it would be good to find a final experiment to better check how having acquired the ability to draw these inferences helps in some more interesting tasks. Or at least that it generalizes to more complex settings}

\tb{We should look at PRONTOQA Saparov and He ICLR 20023}

\tb{\cite{yang:llm24}  Strong evidence of multi-hope reasoning second hop moderate}

\tb{\cite{yang:llm24} study implicit multihop}

\tb{OR more complex linguistic statements: if we manipulate the text to enrich its linguistic complexity eg adding adjectives, or adverbs or composed words does the model still manage to derive inferences properly?}


==> dataset_old.tex <==
\section{Dataset}
\label{sec:data}

Syllogisms consist of two premises and a conclusion that share the
structure ``Quantifier Noun-1 verb Noun-2''; such statements can be in
four \emph{moods}: either affirmative or negative, and either
universal or existential based on the type of quantifier; they are abbreviated using
letters -- affirmatives as ``A'' and ``I'', negatives as ``E'' and ``O'' from
the Latin ``AffIrmo'' and ``nEgO'', respectively. Examples of each
type are in Figure~\ref{fig:ex}. The order in
which the nouns occur within the premises defines the \emph{figure}; there are four
possible figures, which are marked
by numbers: figure 1 has the A-B, B-C order,  the
others are B-A, C-B (figure 2), A-B, C-B (figure 3), and B-A, B-C (figure 4).

Since each premise can be in one of the four moods, there are 64
distinct pairs of premises (16 moods x 4 figures).
%Given this, the total combinations of premises is 64, since each of the two
%premises can appear in four different moods and there are four
%possible figures (4 x 4 x 4). 
We follow the psychology literature and consider 37 of these
combinations as invalid (no conclusion follows), while the remaining 27 lead to at least one 
conclusion. In each syllogism, one premise relates the terms A and B,
and the other relates the terms B and C. Instead, the conclusions
always relate the terms A and C.  Since each of the four moods expresses
an asymmetric relation between two terms, there are always eight possible conclusions
relating the terms A and C.
%\footnote{Note,  "Some A is C" is  different from "Some C is A".}


\paragraph{Task}  
Following~\citet{ragni:when19,eisape:syst23}, we use the
multiple-choice setting. The model is given two premises and nine possible conclusions, including 
the label ``nothing follows''; the latter are given each time in different random order. The model has to generate at least one valid conclusion. 

%Starting from the terms used
%in~\citet{eisape:syst23},  

\paragraph{Believable and Unbelievable Sets} 
Since we are interested in comparing learning methods on the content-effect bias, similarly to~\citet{dsgupta:lang22}, we use triples of
terms ontologically related; we manually generated 10 triples and the 
schemas for one triple, then we automatized the process to the other
triples; we create test sets of syllogisms that are consistent with world knowledge
(believable) or violate it (unbelievable) - in particular we make sure that the valid conclusions are false based on real-world knowledge. For instance, the
triple ``labradors'', ``dogs'', ``canines'' generates the believable
syllogism in~Figure~\ref{fig:ex} (top) and the unbelievable one:
\emph{P1. All labradors are dogs. P2: No canine are labradors. C:
  Some dogs are not canines''}. Each set consists of 640 data points
(64 schemas instantiated with 10 triples of terms). \lb{Further details are in the Supplementary Material (SM).}

These sets are used as test-sets, while the training sets are obtained by replacing words with pseudo-words as described below.

\paragraph{Training sets}  We created the training sets by replacing nouns with pseudo-words. We use 4k
pseudo-words\footnote{We use the gibberish Python library.} and obtain
inferences that respect the form of the original data point but have nonsense content. 
For each reasoning schema, we generated 
$n$-modifications containing either 1 modified instance or  the concatenations of 
$k$-modified instances.  Following this procedure, we build, for each k-setting (1, 4, 8-examples),
$n$-versions of the same dataset; we use each of these versions as an
episode for DFT; the exact same data used to train DFT are used to build the
vector DB exploited by RAG for in-context learning. For SFT we build one dataset
containing all the schema instantiated with pseudo-words 
and models are fine-tuned on it for $n$-epochs. From the 64 syllogisms, we generated 500
versions of each reasoning schema obtaining 32.000
modifications for each k-example setting. 

\tb{Add Fig 2 of the original paper, but with syllogisms instead of fracas}
